Evaluating ChatGPT's Information Extraction Capabilities: An Assessment of Performance, Explainability, Calibration, and Faithfulness

The capability of Large Language Models (LLMs) like ChatGPT to comprehend user intent and provide reasonable responses has made them extremely popular lately. In this paper, we focus on assessing the overall ability of ChatGPT using 7 fine-grained information extraction (IE) tasks. Specially, we present the systematically analysis by measuring ChatGPT's performance, explainability, calibration, and faithfulness, and resulting in 15 keys from either the ChatGPT or domain experts. Our findings reveal that ChatGPT's performance in Standard-IE setting is poor, but it surprisingly exhibits excellent performance in the OpenIE setting, as evidenced by human evaluation. In addition, our research indicates that ChatGPT provides high-quality and trustworthy explanations for its decisions. However, there is an issue of ChatGPT being overconfident in its predictions, which resulting in low calibration. Furthermore, ChatGPT demonstrates a high level of faithfulness to the original text in the majority of cases. We manually annotate and release the test sets of 7 fine-grained IE tasks contains 14 datasets to further promote the research. The datasets and code are available at https://github.com/pkuserc/ChatGPT_for_IE.

==> 1-intro.tex <==
\section{Introduction}

Large Language Models (LLMs) (e.g., GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20}, LaMDA~\cite{DBLP:journals/corr/abs-2201-08239} and PaLM~\cite{DBLP:journals/corr/abs-2204-02311}, etc.) have greatly promoted the development of the Natural Language Processing (NLP) community. With a proper instruction (often the task definition)~\cite{DBLP:journals/corr/abs-2203-02155,DBLP:journals/corr/abs-2205-11916,chung2022scaling,DBLP:conf/emnlp/WangMAKMNADASPK22} and the chain-of-thought (CoT) prompting~\cite{DBLP:journals/corr/abs-2201-11903}, LLMs achieve surprisingly good performances when dealing with unseen tasks. %The zero-shot ability brings humans closer to achieving strong artificial general intelligence (AGI)~\cite{DBLP:journals/jagi/Goertzel14}.

\iffalse
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \resizebox{0.5\textwidth}{!}{
    \includegraphics{figs/relation.pdf}
    }
    \caption{An illustration of each augmentation method's advantages.}
    \label{fig:relation}
    \vspace{-3mm}
\end{wrapfigure}
\fi

ChatGPT~\footnote{https://chat.openai.com/} is currently the most popular LLM, known for its impressive ability to understand user intent and generate human-like responses. ChatGPT is trained on the GPT family~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20,DBLP:conf/emnlp/ArtetxeBGMOSLDI22,DBLP:journals/corr/abs-2203-02155} using reinforcement learning from human feedback
(RLHF)~\cite{DBLP:conf/nips/ChristianoLBMLA17} and high-quality conversational-style datasets. Apart from its surprising dialogue ability, ChatGPT has many other aspects that attract researchers to explore. Some researcher have delved into the potential impacts of ChatGPT on human life~\cite{DBLP:journals/corr/abs-2212-05856,DBLP:journals/corr/abs-2301-12867,DBLP:journals/corr/abs-2212-09292,DBLP:journals/corr/abs-2302-04536}. Other researchers are interested in exploring the capabilities of ChatGPT for various NLP tasks~\cite{DBLP:journals/corr/abs-2212-14548,qin2023chatgpt,DBLP:journals/corr/abs-2301-13852,DBLP:journals/corr/abs-2301-07597}. The capabilities of ChatGPT have been preliminarily explored through the above research and valuable conclusions have been drawn.

Given ChatGPT is a closed model that does not provide information about its training details, and any response from the model encodes an opinion. The response can significantly impact the user’s experience and shape their beliefs going forward~\cite{aiyappa2023can,santurkar2023whose,deshpande2023toxicity,DBLP:journals/corr/abs-2302-07736}. Consequently, evaluating ChatGPT should involve not only assessing its ability to achieve high performance but also measuring the reliability of the answers it provides. To help users better understand the overall quality of ChatGPT’s responses and enable systematic measurement of its capabilities, we design the following four metric dimensions: The first dimension we consider is \textbf{Performance}, which reflects ChatGPT's overall performance on various IE tasks from multiple perspectives. The second metric dimension, \textbf{Explainability}~\cite{DBLP:conf/acl/RajaniMXS19,DBLP:conf/acl/AghajanyanGZ20,DBLP:journals/csur/ZiniA23}, evaluates whether ChatGPT could give a justified reason for its prediction, thereby providing insights into ChatGPT's decision-making process. The third one is \textbf{Calibration}~\cite{DBLP:conf/icml/GuoPSW17,DBLP:conf/nips/KumarLM19,DBLP:conf/nips/ThulasidasanCBB19,DBLP:conf/nips/MindererDRHZHTL21}, which measures the predictive uncertainty of a model, and we use this metric to assess if ChatGPT is overconfidence on its prediction. The last dimension is \textbf{Faithfulness}~\cite{DBLP:conf/acl/MaynezNBM20,koto2022can,DBLP:journals/corr/abs-2208-14271,DBLP:journals/corr/abs-2301-00303}, it is frequently employed in the summarization task to determine whether the summary accurately reflects the input. In our research, we adopt faithfulness as a measure of whether the explanations given by ChatGPT are truthful to the input, or if they are spurious. In summary, according to the above four dimensions, we collect 15 keys from either the ChatGPT or domain experts for the evaluation  (\S~\ref{sec:data_collection}).


In this research, we aim to perform a comprehensive study and detailed analysis of ChatGPT's capabilities through various information extraction (IE) tasks. IE involves heterogeneous structure extraction, factual knowledge usage, and diversified targets\cite{DBLP:conf/emnlp/YamadaASTM20,DBLP:conf/iclr/PaoliniAKMAASXS21,lu-etal-2022-unified}, making it an ideal scenario for evaluating ChatGPT's capabilities. Overall, we conduct our experiments and analysis based on 14 datasets belonging to 7 fine-grained IE tasks(\S~\ref{sec:main}). Additionally, we assess the explainability, calibration, and faithfulness of ChatGPT's responses through both \textit{self-check} and \textit{human-check} (\S~\ref{sec:analysis}). To sum up, our main contributions are summarized as follows:

\begin{itemize}
    \item To assess the overall ability of ChatGPT, we employ a comprehensive and systematic evaluation from four dimensions: 1) performance, 2) explainability, 3) calibration, and 4) faithfulness. We then collected 15 keys belonging to above dimensions from either the ChatGPT or domain experts for the research. All the manually annotated datasets and code are made public available for future research.

    \item We comprehensively evaluate the overall performance of ChatGPT on various tasks in both Standard-IE and OpenIE settings, and compare it with other popular models. Our research indicates that ChatGPT’s performance is not satisfactory in the Standard-IE setting. However, we show that it provides surprisingly good results in the OpenIE setting, as confirmed by human evaluation. Furthermore, we also discover that ChatGPT provides high-quality and trustworthy explanations for its decisions. Although, it displays overconfidence in its predictions, leading to low calibration. Besides, ChatGPT is largely faithful to the original text in most cases. 
\end{itemize}


==> 2-related_work.tex <==
\section{Related Work}

\subsection{Large Language Models}

Large Language Models (LLMs) typically contain more than a hundred billion parameters, such as GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20}, Gopher~\cite{DBLP:journals/corr/abs-2112-11446}, LaMDA~\cite{DBLP:journals/corr/abs-2201-08239}, Megatron-turing-NLG~\cite{DBLP:journals/corr/abs-2201-11990}, and PaLM~\cite{DBLP:journals/corr/abs-2204-02311}, among others. Scaling up the model size brings impressive abilities on few-shot and zero-shot learning scenarios, such as producing reasonable results with very few samples or task descriptions \cite{DBLP:conf/nips/BrownMRSKDNSSAA20,DBLP:journals/corr/abs-2204-02311}. Moreover, scaling up the model size unlocks emergent abilities that were not observed in smaller models, enabling LLMs to exhibit strong generalizability on unseen tasks~\cite{DBLP:journals/corr/abs-2206-07682,fu2022does,DBLP:journals/corr/abs-2301-06627}.

%In zero-shot and few-shot learning scenarios where fine-tuning isn't possible, two approaches can leverage LLMs' capabilities. The first is to provide proper instructions or task descriptions to guide LLMs' output~\cite{DBLP:journals/corr/abs-2203-02155,DBLP:journals/corr/abs-2205-11916,chung2022scaling,DBLP:conf/emnlp/WangMAKMNADASPK22}. The second, called In-Context Learning (ICL), concatenates training samples with input to enable LLMs to better handle new tasks, without gradient updates~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20,DBLP:conf/emnlp/HoltzmanWSCZ21,DBLP:conf/naacl/RubinHB22,DBLP:conf/emnlp/MinLHALHZ22}.

With its impressive ability to understand user intent and generate human-like responses, ChatGPT has become the most popular language model currently. It is trained on the GPT family~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20,DBLP:conf/emnlp/ArtetxeBGMOSLDI22,DBLP:journals/corr/abs-2203-02155} and high-quality conversational-style datasets using reinforcement learning from human feedback (RLHF)~\cite{DBLP:conf/nips/ChristianoLBMLA17}. Along with its dialogue ability, ChatGPT has other aspects that researchers are exploring. Some researchers show potential impacts of ChatGPT on human life, such as ethical risks~\cite{DBLP:journals/corr/abs-2212-05856,DBLP:journals/corr/abs-2301-12867,DBLP:journals/corr/abs-2301-07098}, the education sector~\cite{DBLP:journals/corr/abs-2212-09292,DBLP:journals/corr/abs-2302-04536,kortemeyer2023could} and the medical scenario~\cite{DBLP:journals/corr/abs-2301-13819,DBLP:journals/corr/abs-2301-10035,DBLP:journals/corr/abs-2212-14882}. Additionally, some researchers are keen to examine the potential of ChatGPT in addressing various natural language processing tasks. For instance, some works have examined ChatGPT's performance in stance detection~\cite{DBLP:journals/corr/abs-2212-14548}, linguistic and sentiment analysis~\cite{susnjak2023applying,ortega2023linguistic}, general NLP tasks~\cite{qin2023chatgpt,bian2023chatgpt,zhong2023can}, and machine translation~\cite{DBLP:journals/corr/abs-2301-08745}. \cite{DBLP:journals/corr/abs-2301-13867} explores the mathematical capabilities of ChatGPT, while \cite{DBLP:journals/corr/abs-2302-04023} proposes an evaluation of ChatGPT on reasoning and other aspects. Additionally, \cite{DBLP:journals/corr/abs-2301-13852,DBLP:journals/corr/abs-2301-07597} investigate the differences between human-written and ChatGPT-generated, and conducted several interesting conclusions.


\subsection{Information Extraction}

Information Extraction (IE) is a long-standing research topic that aims to extract structured factual information from unstructured texts~\cite{DBLP:conf/anlp/AndersenHWHSN92,crowe-1995-constraint,chieu-etal-2003-closing,wu-weld-2010-open,khot-etal-2017-answering,lu-etal-2022-unified}. Typically, IE involves a wide range of tasks, such as named entity recognition(NER)~\cite{DBLP:conf/acl/GregoricBC18,DBLP:conf/acl/MartinsMM19,li-etal-2020-unified,DBLP:conf/acl/DasKPZ22}, entity typing(ET)~\cite{DBLP:conf/acl/LevyZCC18,DBLP:conf/acl/DaiSW20,DBLP:conf/acl/PangZZW22,DBLP:conf/acl/0019CJLZ0X22}, relation extraction(RE)~\cite{DBLP:conf/acl/LiYSLYCZL19,DBLP:conf/acl/FuLM19,DBLP:conf/acl/BianHHZZ21,DBLP:conf/acl/YeL0S22}, relation classification(RC)~\cite{zeng2015distant,DBLP:conf/acl/YeLXSCZ19,DBLP:journals/corr/abs-2102-01373,DBLP:journals/corr/abs-2212-14266}, event detection(ED)~\cite{DBLP:conf/acl/VeysehLDN20,DBLP:conf/acl/LouLDZC20,DBLP:conf/acl/LiuCX22,DBLP:conf/emnlp/ZhaoJ0GC22}, event argument extraction(EAE)~\cite{DBLP:conf/emnlp/ZhangSH22,DBLP:conf/emnlp/DuJ22,DBLP:conf/acl/MaW0LCWS22}, and event extraction(EE)~\cite{DBLP:conf/emnlp/WaddenWLH19,DBLP:conf/emnlp/DuC20,DBLP:conf/acl/LiuHSW22,DBLP:conf/naacl/HsuHBMNCP22}, among others. These tasks automatically generate structured factual outputs related to entity, relation and event, and greatly boost the developments of NLP community.

%We choose IE in this research because it involves various knowledge-intensive and complex tasks, including heterogeneous structures extraction (e.g., span identification and triplet extraction), intra- and inter-knowledge usage, and diversified targets (e.g., entity, relation and event)~\cite{DBLP:conf/emnlp/YamadaASTM20,DBLP:conf/iclr/PaoliniAKMAASXS21,lu-etal-2022-unified}. Such features make IE an ideal task for assessing the ability of ChatGPT in scenarios that require the usage of complex reasoning abilities and factual knowledge. In addition, as far as we know, there is currently no large-scale and systematic research on the ability of ChatGPT in the IE field, nor in-depth analysis of the output results.



==> 3-data_collection.tex <==
\section{ChatGPT for Information Extraction}\label{sec:data_collection}
In this section, we first briefly introduce 7 fine-grained IE tasks, then we present how to collect 15 keys from the ChatGPT and domain experts.

\subsection{Information Extraction}

IE involves a wide range of tasks which need to extract structured factual information from unstructured texts, such as entity, relation and event. In this research, we conduct our analysis on the followings 7 fine-grained IE tasks:\footnote{We introduce these tasks briefly due to the space limitation. Please refer to the task-specific papers for more details.} 1) \textbf{Entity Typing(ET)}~\cite{DBLP:conf/acl/LevyZCC18,DBLP:conf/acl/DaiSW20,DBLP:conf/acl/PangZZW22,DBLP:conf/acl/0019CJLZ0X22} aims to classify the type of a target entity under a given input; 2) \textbf{Named Entity Recognition(NER)}~\cite{DBLP:conf/acl/GregoricBC18,DBLP:conf/acl/MartinsMM19,li-etal-2020-unified,DBLP:conf/acl/DasKPZ22} aims to first identify the candidate entities, and then classify their types; 3) \textbf{Relation Classification(RC)}~\cite{zeng2015distant,DBLP:conf/acl/YeLXSCZ19,DBLP:journals/corr/abs-2102-01373,DBLP:journals/corr/abs-2212-14266} requires to classifying the relation between two target entities; 4) \textbf{Relation Extraction(RE)}~\cite{DBLP:conf/acl/LiYSLYCZL19,DBLP:conf/acl/FuLM19,DBLP:conf/acl/BianHHZZ21,DBLP:conf/acl/YeL0S22} is a task that needs to identify the target entities and the relation jointly; 5) \textbf{Event Detection(ED)}~\cite{DBLP:conf/acl/VeysehLDN20,DBLP:conf/acl/LouLDZC20,DBLP:conf/acl/LiuCX22,DBLP:conf/emnlp/ZhaoJ0GC22} identifies event triggers and their types; 6) \textbf{Event Argument Extraction(EAE)}~\cite{DBLP:conf/emnlp/ZhangSH22,DBLP:conf/emnlp/DuJ22,DBLP:conf/acl/MaW0LCWS22} distinguishes arguments and categorizes their roles with respect to the targe event; and 7) \textbf{Event Extraction(EE)}~\cite{DBLP:conf/emnlp/WaddenWLH19,DBLP:conf/emnlp/DuC20,DBLP:conf/acl/LiuHSW22,DBLP:conf/naacl/HsuHBMNCP22} performs event detection and argument
extraction jointly. Note that although some of these tasks are subsets of others, every task needs LLMs' unique ability to perform well. It is worth to explore the performances on these fine-grained IE tasks.

\subsection{Standard-IE Setting and OpenIE Setting}

To comprehensively evaluate the overall performance of ChatGPT on IE tasks, we ask ChatGPT to generate the response from the \textbf{Standard-IE} setting and the \textbf{OpenIE} setting. The Standard-IE setting is commonly used in previous works, which uses the task-specific dataset with supervised learning paradigm to fine-tune a model. For ChatGPT, as we can not directly fine-tune the parameters, we explore evaluating the ChatGPT's ability to select the most appropriate answer from a set of candidate labels instead. Specifically, this setting is based on an instruction that includes the task description, the input text, the prompt and the label set. Where the task description describes the specific IE task, the prompt involves the utterances that guide the ChatGPT outputs the required keys (which will be introduced in \S~\ref{sec:keys}),  and the label set contains all candidate labels based on each dataset. The \textbf{OpenIE} setting is a more advanced and challenging scenario than \textbf{Standard-IE} setting. In this setting, we do not provide any candidate labels to ChatGPT and rely solely on its ability to comprehend the task description, the prompt and input text to generate predictions. Our goal is to assess the ChatGPT's ability to produce reasonable factual knowledge.


\begin{table*}[]
\centering
\setlength{\tabcolsep}{0.6mm}
\begin{tabular}{cl}
\toprule[1.5pt]
\multicolumn{1}{c|}{\textbf{Keys}}                    & \multicolumn{1}{c}{\textbf{Explanation}}                                 \\ \hline
\multicolumn{2}{l}{\textit{\textbf{Performance}}}                                                                                \\ \hline
\multicolumn{1}{c|}{\texttt{Open}}                           & Directly ask ChatGPT to predict the class without the label set.                  \\
\multicolumn{1}{c|}{\texttt{Standard}}                         & ChatGPT’s most likely correct class with a given label set. \\
\multicolumn{1}{c|}{\texttt{Top3}}                             & The three most likely classes of the given label set from ChatGPT.                 \\
\multicolumn{1}{c|}{\texttt{Top5}}                             & The five most likely classes of the given label set from ChatGPT.                  \\
\multicolumn{1}{c|}{\texttt{ifOpen\_Correct(Manual)}}             & Manually annotate whether the "\texttt{Open}" is reasonable.             \\ \hline
\multicolumn{1}{l|}{\textit{\textbf{Explainability}}} &                                                                          \\ \hline
\multicolumn{1}{c|}{\texttt{Reason\_Open}}                      & The reason why ChatGPT chooses the class in "\texttt{Open}".                   \\
\multicolumn{1}{c|}{\texttt{Reason\_Standard}}                      & The reason why ChatGPT chooses the class in "\texttt{Standard}".                 \\ 
\multicolumn{1}{c|}{\texttt{ifR\_Open}}                         & Does ChatGPT think that "\texttt{Reason\_Open}" is reasonable?            \\
\multicolumn{1}{c|}{\texttt{ifR\_Standard}}                         & Does ChatGPT think that "\texttt{Reason\_Standard}" is reasonable?          \\ 
\multicolumn{1}{c|}{\texttt{ifR\_Open(Manual)}}                & Manually annotate whether the "\texttt{Reason\_Open}" is reasonable.                    \\
\multicolumn{1}{c|}{\texttt{ifR\_Standard(Manual)}}                 & Manually annotate whether the "\texttt{Reason\_Standard}" is reasonable.             \\      
\hline
\multicolumn{1}{l}{\textit{\textbf{Calibration}}}     &                                                                          \\ \hline
\multicolumn{1}{c|}{\texttt{Confidence\_Open}}                          & The confidence of ChatGPT in predicting "\texttt{Open}".                                       \\
\multicolumn{1}{c|}{\texttt{Confidence\_Standard}}                          & The confidence of ChatGPT in predicting "\texttt{Standard}".                                     \\ \hline
\multicolumn{1}{l}{\textit{\textbf{Faithfulness}}}    &                                                                          \\ \hline
\multicolumn{1}{c|}{\texttt{FicR\_Open(Manual)}}           & Manually annotate whether the "\texttt{Reason\_Open}" is fictitious.                    \\
\multicolumn{1}{c|}{\texttt{FicR\_Standard(Manual)}}           & Manually annotate whether the "\texttt{Reason\_Standard}" is fictitious.                    \\ \bottomrule[1.5pt]
\end{tabular}
\caption{We gather 15 keys in this research, consisting of 10 keys automatically generated by ChatGPT and 5 keys that required manual annotation (denoted as \texttt{Manual}). These keys provide insight into ChatGPT's ability in four dimensions, namely: 1) performance, 2) explainability, 3) calibration, and 4) faithfulness.}
\label{table:key}
\end{table*}

\subsection{Collecting Keys From ChatGPT And Human Annotation}\label{sec:keys}

In this subsection, we first describe 15 keys that are collected from the ChatGPT and domain experts. In Table~\ref{table:key}, we show 10 keys that are extracted from ChatGPT and 5 keys that need human involvements. These keys could systemically assess ChatGPT's ability from the following four aspects: 

\textbf{Performance.} One important aspect of our research is to comprehensively evaluate the overall performance of ChatGPT on various tasks and compare it with other popular models. By examining its performance from different aspects, we seek to provide a detailed understanding of ChatGPT's capability on the downstream IE tasks. 
    
\textbf{Explainability.} The explainability of ChatGPT is crucial for its application in real-world scenarios~\cite{DBLP:conf/acl/RajaniMXS19,DBLP:conf/acl/AghajanyanGZ20,DBLP:journals/csur/ZiniA23}. In our study, we will measure both the \textit{self-check} and \textit{human-check} explainability of ChatGPT, with a focus on its ability to provide useful and accurate explanations of its reasoning process for humans. Specially, we ask ChatGPT to provide reasons for its predictions (\texttt{Reason\_Open} and \texttt{Reason\_Standard}), and if ChatGPT approves its explanations (\texttt{ifR\_Open} and \texttt{ifR\_Standard}). Additionally, we also manually evaluate the acceptability of these reasons to humans (\texttt{ifR\_Open(Manual)} and \texttt{ifR\_Standard(Manual)}).
    
\textbf{Calibration.} Measuring the calibration helps to evaluate the predictive uncertainty of a model~\cite{DBLP:conf/icml/GuoPSW17,DBLP:conf/nips/KumarLM19}. A properly calibrated classifier should have predictive scores that accurately reflect the probability of correctness~\cite{DBLP:conf/nips/ThulasidasanCBB19,DBLP:conf/nips/MindererDRHZHTL21}. Given the tendency of modern neural networks to be overconfident in their predictions, we aim to identify potential uncertainties or overconfidence phenomenon of ChatGPT. To evaluate the calibration, ChatGPT is required to provide a confidence score (ranging from 1 to 100) for each prediction it makes (\texttt{Confidence\_Open} and \texttt{Confidence\_Standard}). 
    %We will also investigate how ChatGPT deals with unexpected or ambiguous input, which can affect its reliability.
    
\textbf{Faithfulness.} The faithfulness of ChatGPT's explanation is important to ensure its trustworthiness~\cite{DBLP:conf/acl/MaynezNBM20,DBLP:journals/corr/abs-2301-00303}. In evaluating the faithfulness, we have included two keys that assess whether the reasons provided by ChatGPT are faithful to the original input. These keys, \texttt{FicR\_Open(Manual)} and \texttt{FicR\_Standard(Manual)}, require manual annotation by domain experts.

Due to the space limitation, we show an intuitive example in the Appendix~\ref{app:input} to help readers better understand the annotation process.

%We show an intuitive example from BBN dataset~\footnote{This is a popular dataset in entity typing task.}~\cite{weischedel2005bbn} to help readers better understand the annotation process. Suppose the given input text is $I$ = \textit{\uline{Silicon Valley heaved a sigh of relief yesterday.}}, and the target is \textit{Silicon Valley}. The input instruction and the ChatGPT's response are show in Figure~\ref{}, where the bold text is input-specific.~\footnote{Please refer to Appendix~\ref{} for more examples on each task.}







==> 4-experiments.tex <==
\section{Performance}\label{sec:main}

\subsection{Setup}
To ensure a comprehensive evaluation of ChatGPT's capabilities, we conduct manual annotation and analysis on a diverse range of IE tasks, including 7 fine-grained tasks spanning 14 datasets. We collected 15 keys for each dataset from both ChatGPT and domain experts (\S~\ref{sec:data_collection}). Only the test sets are annotated, as our aim is to analysis ChatGPT's abilities without any training. For space reasons, the detail of each dataset is shown in the Appendix~\ref{app:data}. Due to the time-consuming nature of obtaining responses from domain experts, we randomly select nearly 3,000 samples in total for our analysis. The number of manually annotated samples for each dataset is reported in the Appendix~\ref{app:data}. As for the outputs from ChatGPT, we use the official API to evaluate the whole test sets.~\footnote{To prevent any historical chat biases, we cleared every conversation after generating each response.} 

Besides, we compare ChatGPT with several popular baselines: 1) \textbf{BERT}~\cite{DBLP:conf/naacl/DevlinCLT19} and \textbf{RoBERTa}~\cite{DBLP:journals/corr/abs-1907-11692}, and 2) \textbf{State-of-the-Art} (SOTA) on the single dataset. Due to the space limitation, the details of state-of-the-art methods are shown in the Appendix~\ref{app:sota}. As for the metric, we use Micro-F1 score for all tasks expect RE and EE. For the RE task, we report the named entity recognition F1-score and the relation classification F1-score. As for the EE task, we show the trigger F1-score and argument F1-score.~\footnote{These metrics are all following previous works.}

\subsection{Performance on the Standard-IE Setting}

In this subsection, we report the performances on the Standard-IE setting, as depicted in Table~\ref{tab:main}. \textbf{It is clear from the table that ChatGPT’s performance is not comparable to that of baseline models and SOTA methods in most cases.} This is not surprising given directly asking ChatGPT for the prediction is more like a zero-shot scenario, whereas the other compared methods are trained on task-specific datasets under a supervised learning paradigm. Nevertheless, ChatGPT can achieve reasonable results in some cases through its user-friendly communication design, demonstrating exceptional generalization capabilities for a wide range of IE tasks.

Besides, our research indicates that \textbf{ChatGPT performs well on relatively simple IE tasks but struggles with more complex and challenging tasks.} For example, the entity typing (ET) task only involves classifying entities into predefined types without any further contextual analysis, and ChatGPT excels at this task, demonstrating that the model can generate accurate factual knowledge when the task is simple. However, in complex and challenging IE tasks such as RE, ChatGPT struggles as it requires first identifying the entities that exist in the input and then classifying the relationship between them, which is a more challenging task than ET. Despite ChatGPT’s acceptable results on the ET, NER and RC tasks, it still faces challenges with more multifaceted IE tasks like RE and EE, where deeper contextual analysis and reasoning abilities are required. In summary, ChatGPT’s performance varies based on the complexity of the task, and it performs well on straightforward tasks.

%Besides, our research indicates that ChatGPT performs well on relatively simple IE tasks but struggles with complex ones. Specially, ChatGPT exhibits the best performance on the entity typing (ET) task and delivers acceptable results on the named entity recognition (NER). This demonstrates that ChatGPT could output correct fact knowledge when the task is straightforward.~\footnote{The ET task is considered straightforward due to its unambiguous nature, as it involves only classifying entities into predefined types without any further contextual analysis.} As for the complex and challenging IE tasks, such as relation extraction (RE) and event extraction (EE),~\footnote{For instance, RE needs to first identify the entities existing in the input, and further classifies the relationship between two entities. This is much harder than directly distinguish the type of a given entity.} ChatGPT faces difficulties to deal with and the performances are disappointing.


Furthermore, the conclusion that ChatGPT performs worse than other models seems inconsistent with previous studies~\cite{DBLP:journals/corr/abs-2302-10205,DBLP:journals/corr/abs-2303-03836}, which suggest that ChatGPT can achieve desirable performance in some IE tasks. One possible explanation for the difference in conclusions is that we report the performance of the entire test set for each task in our study, while prior studies reported on a very small set of test samples drawn at random, which may have substantial variance. Another factor may be that we used a concise and relatively unified prompt to guide ChatGPT, while other research relied on domain-specific prompts or included a large number of label descriptions in their prompts, which needs lots of domain knowledge and thereby limits the ability to generalize across various tasks.



\begin{table*}[]
\setlength{\tabcolsep}{1.0mm}
\begin{tabular}{c|c|c|c|c|c}
\toprule[1.5pt]
\textbf{Task}                                                                                          & \textbf{Dataset}              & \textbf{BERT} & \textbf{RoBERTa} & \textbf{SOTA} & \textbf{ChatGPT}  \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Typing(ET)\end{tabular}}}              & \textbf{BBN}           & 80.3          & 79.8             & 82.2~\cite{DBLP:conf/coling/ZuoLJZFL22}          &     85.6       \\ \cline{2-2}
                                                                                                   & \textbf{OntoNotes 5.0} & 69.1          & 68.8             & 72.1~\cite{DBLP:conf/coling/ZuoLJZFL22}          &  73.4                      \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Named Entity\\ Recognition(NER)\end{tabular}}}  & \textbf{CoNLL2003}     & 92.8          & 92.4             & 94.6~\cite{DBLP:conf/acl/WangJBWHHT20a}          & 67.2             \\ \cline{2-2}
                                                                                                   & \textbf{OntoNotes 5.0} & 89.2          & 90.9             & 91.9~\cite{DBLP:conf/acl/YeL0S22}          & 51.1            \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Relation\\ Classification(RC)\end{tabular}}}    & \textbf{TACRED}        & 72.7      & 74.6             & 75.6~\cite{DBLP:journals/corr/abs-2212-14270}          & 20.3             \\ \cline{2-2}
                                                                                                   & \textbf{SemEval2010}   & 89.1          & 89.8             & 91.3~\cite{DBLP:journals/kbs/ZhaoXCLG21}          & 42.5  \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Relation\\ Extraction(RE)\end{tabular}}}        & \textbf{ACE05-R}       & 87.5 | 63.7     & 88.2 | 65.1        &    91.1 | 73.0~\cite{DBLP:conf/acl/YeL0S22}    & 40.5 | 4.5        \\ \cline{2-2}
                                                                                                   & \textbf{SciERC}        & 65.4 | 43.0     & 63.6 | 42.0        &  69.9 | 53.2~\cite{DBLP:conf/acl/YeL0S22}    & 25.9 | 5.5       \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Event\\ Detection(ED)\end{tabular}}}            & \textbf{ACE05-E}       & 71.8          &     72.9     & 75.8~\cite{DBLP:conf/acl/LiuCX22}          & 17.1         \\ \cline{2-2}
                                                                                                   & \textbf{ACE05-E+}      & 72.4          & 72.1          & 72.8~\cite{DBLP:conf/acl/LinJHW20}          & 15.5          \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Event Argument\\ Extraction(EAE)\end{tabular}}} & \textbf{ACE05-E}       & 65.3          &    68.0       & 73.5~\cite{DBLP:conf/naacl/HsuHBMNCP22}          & 28.9           \\ \cline{2-2}
                                                                                                   & \textbf{ACE05-E+}      & 64.0          &  66.5         & 73.0~\cite{DBLP:conf/naacl/HsuHBMNCP22}          & 30.9   \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Event\\ Extraction(EE)\end{tabular}}}           & \textbf{ACE05-E}       & 71.8 | 51.0     &   72.9 | 51.9       & 74.7 | 56.8~\cite{DBLP:conf/acl/LinJHW20}     & 17.0 | 7.3         \\ \cline{2-2}
                                                                                                   & \textbf{ACE05-E+}      & 72.4 | 52.7     &   72.1 | 53.4      & 71.7 | 56.8~\cite{DBLP:conf/naacl/HsuHBMNCP22}     & 16.6 | 7.8      \\\bottomrule[1.5pt]
\end{tabular}
\caption{The performances of ChatGPT and several baseline models on 14 IE datasets on the Standard-IE setting. We report the performance on the whole test set. All results are directly cited from public papers or re-implemented using official open-source code.}
\label{tab:main}
\end{table*}



\begin{table}[]
\centering
\setlength{\tabcolsep}{2.0mm}
\begin{tabular}{c|c|c}
\toprule[1.5pt]
           & \textbf{Standard-IE} & \textbf{OpenIE} \\ \hline
\textbf{BBN}(\textit{ET})     & 86.8\%                      & 97.2\%                    \\
\textbf{CoNLL}(\textit{NER})  &  69.0\%                   & 93.3\%                    \\
\textbf{SemEval2010}(\textit{RC}) & 43.3\%                  & 84.3\%                    \\
\textbf{ACE05-R}(\textit{RE}) &   14.9\%                    & 23.9\%                    \\
\textbf{ACE05-E}(\textit{ED})  & 12.4\%                      & 42.6\%                    \\
\textbf{ACE05-E}(\textit{EAE}) & 17.3\%                      & 65.3\%                    \\
\textbf{ACE05-E}(\textit{EE})  & 4.9\%                       & 28.8\%                    \\ \bottomrule[1.5pt]
\end{tabular}
\caption{The accuracy of Standard-IE setting and OpenIE setting on the sampled test set. Our results show that ChatGPT could generate reasonable outputs on the OpenIE setting.}\label{tab:open}
\end{table}

\subsection{Performance on the OpenIE Setting} 

In this subsection, we report both the accuracy of Standard-IE setting and OpenIE setting on the sampled dataset.~\footnote{We randomly selected around 200 samples for each dataset.} For the Standard-IE setting, we provide the pre-defined label set and ask the ChatGPT to choose an answer for a given input, and the accuracy was calculated by matching the predictions to the ground truth labels. On the other hand, the OpenIE setting refers to asking ChatGPT to make predictions without the pre-defined label set (\texttt{Open} in \S~\ref{sec:keys}). Three domain experts evaluate these predictions and vote on whether they were reasonable in light of the input and background knowledge, named as \texttt{ifOpen\_Correct} in \S~\ref{sec:keys}. Our main goal is to determine if ChatGPT could produce logical and reasonable predictions without given the pre-defined label set, so we do not require the prediction match the ground truth. 

The results presented in Table~\ref{tab:open} indicate that \textbf{ChatGPT’s performance is somewhat inspiring under the OpenIE setting}. For example, more than 84\% of the predictions are considered reasonable by the domain experts in ET, NER, and RC tasks. However, the performance is relatively poorer for more challenging tasks, such as RE and EE. Overall, compared with Standard-IE setting, ChatGPT's performance on the OpenIE setting is exciting. Our findings suggest that under the OpenIE setting, ChatGPT could generate reliable factual knowledge and reasonable output for less complex questions. 



\begin{table*}[h]
\centering
\setlength{\tabcolsep}{2.0mm}
\begin{tabular}{c|ccc|ccc}
\toprule[1.5pt]
\multirow{2}{*}{}    & \multicolumn{3}{c|}{\textbf{Stardand Setting}}                          & \multicolumn{3}{c}{\textbf{OpenIE Setting}}                             \\ \cline{2-7} 
                     & \textbf{Self-check} & \textbf{Human-check} & \textbf{Overlap} & \textbf{Self-check} & \textbf{Human-check} & \textbf{Overlap} \\ \hline
\textbf{BBN} (\textit{ET})        & 100.0\%                & 99.2\%                   & 99.2\%              & 100.0\%                & 99.5\%                   & 99.5\%              \\
\textbf{CoNLL} (\textit{NER})   & 100.0\%                & 99.3\%                   & 99.3\%              & 100.0\%                 & 99.7\%                   & 99.7\%              \\
\textbf{SemEval} (\textit{RC}) & 100.0\%                & 100.0\%                  & 100.0\%             & 100.0\%                & 99.7\%                   & 99.7\%              \\
\textbf{ACE05-R} (\textit{RE})  & 100.0\%                & 90.0\%                   & 90.0\%              & 100.0\%                & 100.0\%                  & 100.0\%             \\
\textbf{ACE05-E} (\textit{ED})  & 100.0\%                & 96.3\%                   & 96.3\%              & 100.0\%                & 90.2\%                   & 90.2\%              \\
\textbf{ACE05-E} (\textit{EAE})   & 100.0\%                & 74.1\%                   & 74.1\%              & 100.0\%                & 90.4\%                   & 90.4\%              \\
\textbf{ACE05-E} (\textit{EE})  & 100.0\%                & 47.1\%                   & 47.1\%              & 94.0\%                 & 78.0\%                   & 74.0\%              \\ \bottomrule[1.5pt]
\end{tabular}
\caption{The explainability of ChatGPT measured on the sampled test set. We report the ratio of samples with reasonable reasons discriminated by ChatGPT (\textit{self-check}) and domain experts (\textit{human-check}) under different settings. Besides, we also compute the overlap ration for both of them. These results indicate that in most cases, ChatGPT exhibits strong explainability for its prediction.}\label{table:reason}
\end{table*}

\subsection{The \textit{top-k} Recall Analysis}

\begin{table}[h]
\centering
\setlength{\tabcolsep}{1.0mm}
\begin{tabular}{c|c|c|c}
\toprule[1.5pt]
\textbf{}            & \textit{\textbf{top-1}} & \textit{\textbf{top-3}} & \textit{\textbf{top-5}} \\ \hline
\textbf{BBN}         & 85.6\%                   & 92.7\%                   & 94.9\% (+9.3\%)                  \\
\textbf{SemEval2010} & 42.5\%                   & 62.1\%                   & 76.0\% (+33.5\%)                  \\\bottomrule[1.5pt]
\end{tabular}
\caption{The \textit{top-k} recall analysis on the whole test set. We report two datasets due to the space limitation, other datasets show similar observation. The results show that ChatGPT could server as a good advisor.}\label{tab:recall}
\end{table}

While generating the most likely prediction may be unsatisfactory on the Standard-IE setting, we seek to investigate whether ChatGPT could be a useful advisor. Therefore, we examine the recall of its \textit{top-k} predictions, with \textit{k} = \textit{1}, \textit{3}, or \textit{5}. As shown in Table~\ref{tab:recall}, the results indicate that compared with the \textit{top-1} recall, the \textit{top-3} recall increases significantly, e.g., the improvement is 19.6\% on SemEval2010. Moreover, the \textit{top-5} recall reaches an impressive 94.9\% on BBN and 76.0\% on SemEval2010, demonstrating a favorable outcome. Our findings suggest that \textbf{ChatGPT is a competent answer candidate generator for a given task under the Standard-IE setting}, which could help users select the most probable prediction from the \textit{top-5} predictions.



%\noindent \textbf{Long-tailed Scenario}

%\noindent \textbf{The Impact of Input Length} Classical deep learning IE methods face significant difficulties with long input lengths since it becomes challenging for models to extract informative information. In this subsection, we investigate whether ChatGPT can overcome this problem. We select three tasks and present their performances based on input length in Figure~\ref{}. Our observations highlight that ChatGPT shows stable performance with increasing input length, whereas RoBERTa exhibits a significant performance reduction, particularly for the XX task.  From the above results we can see that ChatGPT is not sensitive to the input length, suggest that it could handle the long input well.






==> 5-analysis.tex <==
\section{Explainability, Calibration and Faithfulness}\label{sec:analysis}
While ChatGPT’s performance in evaluations is noteworthy, it is equally important to evaluate its ability from diverse dimensions that could offer important insights for future research directions. In this section, we analyze several relevant factors, including explainability, calibration, and faithfulness, to comprehensively evaluate ChatGPT’s abilities. Overall, our findings suggest that ChatGPT provides high-quality and reliable explanations for its predictions, but it tends to display overconfidence in most cases, leading to low calibration. Additionally, ChatGPT displays high faithfulness to the original text, making it an reliable tool for users.

\subsection{Explainability}

Explainability is a critical requirement for LLMs, as it enables users to understand how the model arrives at its predictions~\cite{DBLP:journals/corr/abs-2302-12813}. In this study, we investigate whether ChatGPT could provide a reasonable explanation for its output. To be specific, we request ChatGPT to provide reasons for its predictions in the Standard-IE and OpenIE settings. The corresponding keys are denoted as \texttt{Reason\_Standard} and \texttt{Reason\_Open}, as explained in \S~\ref{sec:keys}. These reasons are then evaluated for their reasonableness by both ChatGPT and three domain experts, with the resulting evaluations referred to as \textit{self-check} and \textit{human-check}, respectively. We only consider the samples with correct predictions in the Standard-IE setting to ensure a robust evaluation of ChatGPT’s explainability ability.~\footnote{We randomly select around 200 samples from each dataset for human annotation.} This is because evaluating the reasons provided by ChatGPT for incorrect predictions is less valuable. 

The ratio of samples with reasonable explanations (termed as \textit{reasonable score}) is summarized in Table~\ref{table:reason}, from which we can observe the following conclusions. Firstly, both \textbf{ChatGPT and domain experts highly approve of the reasons given by ChatGPT}, with the majority of datasets achieving a \textit{reasonable score} of over 90\% in the Standard-IE and OpenIE settings. The above results demonstrate that ChatGPT gives very high-quality explanation for its prediction. Secondly, we observe that \textbf{ChatGPT displays a high level of confidence in the reasons provided for its predictions when compared with human evaluation}. In fact, ChatGPT achieves nearly a 100\% \textit{reasonable score} among almost all datasets. This suggests that ChatGPT is very confident in its ability to provide reasonable explanations. Thirdly, we find that \textbf{when ChatGPT provides a reasonable explanation for a prediction, there is a high level of agreement between ChatGPT and human evaluations}. This suggests that ChatGPT may have a similar understanding of explanations as humans. Overall, our findings suggest that ChatGPT is capable of providing high-quality, reliable explanations for its predictions. This is a crucial step towards developing trust and reliability LLMs.

\begin{table*}[]
\centering
\setlength{\tabcolsep}{3.0mm}
\begin{tabular}{c|ccc|ccc}
\toprule[1.5pt]
                      & \multicolumn{3}{c|}{\textbf{Correct Confidence}}                        & \multicolumn{3}{c}{\textbf{Incorrect Confidence}}                           \\ \cline{2-7} 
                      & \multicolumn{1}{c}{\textbf{BERT}} & \textbf{RoBERTa} & \textbf{ChatGPT} & \textbf{BERT} & \multicolumn{1}{c}{\textbf{RoBERTa}} & \textbf{ChatGPT} \\ \hline
\textbf{BBN}\textit{(ET)}      &           0.971               &    0.968        & 0.888            &   0.904      &    0.885                             & 0.828            \\
\textbf{CoNLL}\textit{(NER)}   &        0.990                &     0.991       & 0.864            &   0.866     &   0.886                             & 0.785            \\
\textbf{SemEval}\textit{(RC)}  &    0.983                        &  0.989            & 0.868            &  0.871         &  0.852                                  & 0.839            \\
\textbf{ACE05-R}\textit{(RE)}  &   0.995                        &    0.991          & 0.760            &  0.883        &  0.810                                & 0.764            \\
\textbf{ACE05-E}\textit{(ED)}  &    0.882                          &  0.944          & 0.852            &  0.770         &  0.871                                & 0.737            \\
\textbf{ACE05-E}\textit{(EAE)} &      0.762                       &  0.785          & 0.956            & 0.525         &  0.555                               & 0.910            \\
\textbf{ACE05-E}\textit{(EE)}  &     0.763                        &  0.782           & 0.845            &  0.612        &  0.628                                & 0.764            \\ \bottomrule[1.5pt]
\end{tabular}
\caption{The prediction confidence of various models on the whole test set. We show both the \textit{correct confidence} and \textit{incorrect confidence} based on various methods. We find that ChatGPT is overconfidence for its prediction in most cases.}\label{tab:confidence}
\end{table*}

\subsection{Calibration}


In this subsection, we first investigate the level of confidence for both the correct and incorrect samples. Confidence is typically described in terms of a probability value, indicating the likelihood of belonging to a specific category. To obtain prediction probabilities from ChatGPT, we ask it to output the probability (\texttt{Confidence\_Standard} and \texttt{Confidence\_Open}), as discussed in \S~\ref{sec:keys}.  Our aim is to investigate whether ChatGPT can provide a reasonable prediction confidence for its predictions, thus reducing the risk of misinterpretation. In Table~\ref{tab:confidence}, we present the confidence scores of correct and incorrect predictions from different models, referred to \textit{correct confidence} and \textit{incorrect confidence}, respectively. Our observations reveal that all the models exhibit high confidence levels in their predictions, this is consistent with previous research on large models~\cite{DBLP:conf/icml/GuoPSW17}. \textbf{Although ChatGPT performs worse than its BERT-based counterparts in Standard-IE setting, it displays overconfidence in both correct and incorrect predictions.} Consequently, this overconfidence could lead to misguidance of users. Furthermore, we note a significant confidence gap between correct and incorrect predictions, indicating the need for careful evaluation when ChatGPT's prediction has relatively low confidence.

\begin{table}[h]
\centering
\setlength{\tabcolsep}{0.8mm}
\begin{tabular}{c|ccc}
\toprule[1.5pt]
                      & \multicolumn{1}{c}{\textbf{BERT}} & \textbf{RoBERTa} & \textbf{ChatGPT} \\ \hline
\textbf{BBN}\textit{(ET)}      &        0.012                 &    0.012          & 0.026            \\
\textbf{CoNLL}\textit{(NER)}   &        0.052                      &    0.044          & 0.204            \\
\textbf{SemEval}\textit{(RC)}  &       0.023                      &   0.031          & 0.460            \\
\textbf{ACE05-R}\textit{(RE)}  &       0.020                     &    0.014       & 0.745            \\
\textbf{ACE05-E}\textit{(ED)}  &      0.161                       &   0.226          & 0.656            \\
\textbf{ACE05-E}\textit{(EAE)} &      0.154                       &   0.168          & 0.699            \\
\textbf{ACE05-E}\textit{(EE)}  &      0.211                        &   0.288           & 0.699            \\ \bottomrule[1.5pt]
\end{tabular}
\caption{The expected calibration error (ECE) is used to measure the calibration of a given model, and the lower, the better. Results are calculated on the whole test set.}\label{tab:calibration}
\end{table}


%We present the results in Table~\ref{tab:confidence}, where we list the confidence values of both the correct and incorrect samples provided by different models, referred to as correct confidence and incorrect confidence, respectively. We observe that: 1) all three models show very high confidence on both correct and incorrect samples, this is in line with previous research that large models tend to show confident to their prediction~\cite{DBLP:conf/icml/GuoPSW17}. However, ChatGPT’s overconfidence is apparent despite its lower performance compared to BERT-based models in standard settings. 2) The incorrect confidence is much lower than the correct confidence with BERT-based models. Nevertheless, ChatGPT exhibits high prediction confidence even when the prediction is incorrect. This overconfidence could lead to some misguidance for users. 3) Moreover, for ChatGPT, we identified a notable distinction between the confidence among incorrect and correct samples, particularly in the \textbf{EAE} task, suggesting the need for careful evaluation of results when ChatGPT’s prediction has relatively low confidence.

%BERT-based models show different confidence under different tasks, while ChatGPT gives a relatively stable prediction confidence among all tasks.

We then focus on calibration, a critical property of LLMs as it could estimate the predictive uncertainty for the secure application of LLMs. A well-calibrated model not only produces accurate predictions but also provides reliable and informative uncertainty estimates, necessary for sound decision-making. In this research, we evaluate the calibration using the Expected Calibration Error (ECE) metric, which measures the deviation between predicted confidence and accuracy.~\footnote{We set the bin size to 50, dividing the prediction probabilities into 50 equally spaced bins for analysis.} The results are shown in Table~\ref{tab:calibration}, we can observe that ChatGPT shows much poorer calibration compared to BERT-based methods, which indicates that \textbf{ChatGPT tends to produce confidences that do not represent true probabilities easily}. Furthermore, although ChatGPT displays low ECE in tasks such as ET and NER, miscalibration phenomenon dominates most cases. These findings suggest that ChatGPT needs improvement in terms of calibration, especially for IE tasks.



\subsection{Faithfulness}

\begin{table}[h]
\centering
\setlength{\tabcolsep}{3.0mm}
\begin{tabular}{c|c|c}
\toprule[1.5pt]
                      & \textbf{Stardand-IE} & \textbf{OpenIE} \\ \hline
\textbf{BBN}(\textit{ET})      & 98.3\%                    & 99.3\%                  \\
\textbf{CoNLL}(\textit{NER})   & 100.0\%                    & 98.7\%                  \\
\textbf{SemEval}(\textit{RC})  & 100.0\%                   & 99.1\%                  \\
\textbf{ACE05-R}(\textit{RE})  & 90.0\%                    & 93.8\%                  \\
\textbf{ACE05-E}(\textit{ED})  & 100.0\%                   & 100.0\%                 \\
\textbf{ACE05-E}(\textit{EAE}) & 100.0\%                   & 96.5\%                  \\
\textbf{ACE05-E}(\textit{EE})  & 100.0\%                   & 97.0\%                  \\ \bottomrule[1.5pt]
\end{tabular}
\caption{The evaluation of faithfulness for ChatGPT. Faithfulness refers to whether ChatGPT’s explanation align with the original text. Experimental results show that ChatGPT’s explanation maintains a very high degree of faithfulness to the original text and provide nearly no false explanation.}\label{tab:faithfulness}
\end{table}

Recent works show that ChatGPT may provide false information to users, potentially affecting their decision-making~\cite{DBLP:journals/corr/abs-2302-07736}. Therefore, assessing the faithfulness of the ChatGPT model to the original text is a crucial measure in developing a trustworthy information extraction model. Our study uses faithfulness as a metric to evaluate the ChatGPT model, specifically referring to if the explanation provided by ChatGPT aligns with the original text when its predictionis correct, as the original text is the most important source for extraction information. There are two keys we collect by domain experts, namely \texttt{FicR\_Standard(Manual)} and \texttt{FicR\_Open(Manual)}, as we mentioned in \S~\ref{sec:keys}. Our results are shown in Table~\ref{tab:faithfulness}, which indicate a high degree of faithfulness between ChatGPT’s explanations and the original text with rare false explanations, i.e., with over 95\% of samples considered faithful in nearly all datasets under different settings. We can conclude that\textbf{ ChatGPT’s decision-making process primarily relies on the input of the original text}, leading to the majority of its explanations being regarded as truthful and reliable.


%\subsection{Is the Label Readability influences ChatGPT's Performance?}


